Optimal Non-Adaptive Tolerant Junta Testing via Local Estimators

We give a non-adaptive algorithm that makes $2^{\tilde{O}(\sqrt{k\log(1/\varepsilon_2 - \varepsilon_1)})}$ queries to a Boolean function $f:\{\pm 1\}^n \rightarrow \{\pm 1\}$ and distinguishes between $f$ being $\varepsilon_1$-close to some $k$-junta versus $\varepsilon_2$-far from every $k$-junta. At the heart of our algorithm is a local mean estimation procedure for Boolean functions that may be of independent interest. We complement our upper bound with a matching lower bound, improving a recent lower bound obtained by Chen et al. We thus obtain the first tight bounds for a natural property of Boolean functions in the tolerant testing model.

==> images/junta.tex <==
%!TEX root = ../tolerant.tex

%\begin{figure}
%
%\begin{tikzpicture}
%	
%\end{tikzpicture}
%
%\caption{Do we want a junta figure as well? \red{{\bf Rocco:} Maybe we're okay without a junta figure?}}
%\label{fig:junta}
%	
%\end{figure}


==> images/monotone-n.tex <==
%!TEX root = ../tolerant.tex
%
%\usetikzlibrary{decorations.pathreplacing,angles,quotes}
%\usetikzlibrary{shapes.geometric}
%\usetikzlibrary{patterns}
%
%\begin{figure}
%
%\centering
%
%\begin{tikzpicture}[scale=0.86]
%
%	%%%%%%%%%%%%%%% CONTROL SUBCUBE %%%%%%%%%%%%%%%%% 
%	
%	% colors
%	\fill[pattern= crosshatch,pattern color=black, opacity=0.25] (-1, -1.5) -- (-0.5, -1) -- (-2.25, 0.75) -- (-2.75, 0.25);
%	\fill[pattern= crosshatch,pattern color=black, opacity=0.25] (1, -1.5) -- (0.5, -1) -- (2.25, 0.75) -- (2.75, 0.25);
%%	\fill[pattern=north west lines,pattern color=black, opacity=0.5] (-0.5, -1) -- (0, -1.5) -- (0.5, -1) -- (0, -0.5);
%	
%	\fill[color=purple!20!blue!40!white!70] (-2.25, 0.75) -- (-0.5, -1) -- (0, -0.5) -- (0.5, -1) -- (2.25, 0.75) -- (0, 3);
%	\fill[color=purple!20!blue!40!white!70] (-2.5, 0.5) -- (0, 3) -- (2.5, 0.5);
%	
%	\fill[color=white] (-3, 0) -- (0, -3) -- (3, 0); 
%	
%	% control cube
%	\draw[-] (0, -3) -- (-3, 0) -- (0, 3) -- (3, 0) -- (0, -3);
%	\draw[dashed] (-3, 0) -- (3, 0);
%	\draw[dashed] (-2.5, 0.5) -- (2.5, 0.5);
%
%	
%	% talagrand subcubes
%	\draw[-] (-2.75, 0.25) -- (-1, -1.5) -- (1.75, 1.25);
%	\draw[-] (-2.25, 0.75) -- (0, -1.5) -- (2.25, 0.75);
%	\draw[-,line width=0.3mm] (-1.75, 1.25) -- (1, -1.5) -- (2.75, 0.25) -- (0,3) -- (-1.75, 1.25);
%		
%	% nodes
%	\node (0) at (0, -2){$0$};
%	\node (1) at (0, 1){$1$};
%	\node (talagrand-cube) at (1.15, -0.85){$\bT_{\ell}$};
%	
%%	\node (blah) at (-3.75, 0){$|x| = \frac{m}{2}$};
%%	\node (bleh) at (-4.25, 0.5){$|x| = \frac{m + 0.1\eps\sqrt{m}}{2}$};
%	
%	\draw[decoration={brace,raise=5pt,}, decorate, line width=0.25mm] (-3.05, 0) -- node[left=2pt, align=center, text width = 2.5cm] {\footnotesize $\sbra{\frac{m}{2}, \frac{m + 0.1\eps\sqrt{m}}{2}}$} (-3.05, 0.5);
%	
%	
%	%%%%%%%%%%%%%%%% ACTION SUBCUBES %%%%%%%%%%%%%%%%%
%	
%	% top
%	
%	\node (heads) at (5.5, 2.5){\includegraphics[width=1.1cm]{images/quarter-front}};
%	\node (bh) at (5.5, 1.5){If $\bb_{\ell} = 1$:};
%	
%	\fill[color=purple!20!blue!40!white!70] (10, 2) -- (9, 1) -- (8, 2);
%	
%	\draw[-] (9, 1) -- (7.5, 2.5) -- (9, 4) -- (10.5, 2.5) -- (9, 1);
%	\draw[dashed] (10, 2) -- (8, 2);
%	\draw[dashed] (10, 3) -- (8, 3);
%	
%	\node() at (9, 3.4){$0$};
%	\node() at (9, 2.5){$0$};
%	\node() at (9, 1.6){$1$};
%	
%	% bottom
%	
%	\node (tails) at (5.5, -2){\includegraphics[width=1.1cm]{images/quarter-back}};
%	\node (bt) at (5.5, -3){If $\bb_{\ell} = 0$:};
%	
%	\fill[color=purple!20!blue!40!white!70] (10, -1.5) -- (9, -0.5) -- (8, -1.5);
%	
%	\draw[-] (9, -3.5) -- (7.5, -2) -- (9, -0.5) -- (10.5, -2) -- (9, -3.5);	
%	\draw[dashed] (10, -2.5) -- (8, -2.5);
%	\draw[dashed] (10, -1.5) -- (8, -1.5);
%	
%	\node() at (9, -1.1){$1$};
%	\node() at (9, -2){$0$};
%	\node() at (9, -2.9){$0$};
%	
%	\draw[decoration={brace,raise=5pt}, decorate, line width=0.25mm] (10.5, 3) -- node[right=2pt, align=center, text width = 2.5cm] {\footnotesize $\sbra{\frac{a}{2} \pm c_1\sqrt{a}}$} (10.5, 2);
%	
%	%%%%%%%%%%%%%%%%%%%% EXTRA GOODIES %%%%%%%%%%%%%%%%
%	
%	\draw[-latex] (2.35, 0.1) -- (4.5, 2.25);
%	\draw[-latex] (2.35, 0.1) -- (4.5, -2.25);
%	\node () at (2.35, 0.1) [circle,fill,inner sep=1pt]{};
%	
%	\node (control) at (0, -4.75){$\zo^{\bC} \equiv \zo^m$};
%	\node (action) at (9, -4.75){$\zo^{\bA} \equiv \zo^{a}$};
%	
%\end{tikzpicture}
%
%\caption*{A draw of $\fno\sim\Dno$.} 
%%\red{{\bf Rocco:} I think given the previous caption we can omit everything but the preceding sentence from this caption? Also, can we get both pictures on the same page? (The pictures look great!)}
%% As before, the left hand side depicts the control subcube with the terms of the Talagrand DNF, and the right hand side depicts the action subcube. The cross-hatched region in the control subcube corresponds to outcomes of the control bits for which the action subcube determines the value of $\fno$, and the dashed lines indicate Hamming levels.}
%%}
%\label{fig:montone-yes}
%	
%\end{figure}
%
%


==> images/monotone-y.tex <==
%!TEX root = ../tolerant.tex

\usetikzlibrary{decorations.pathreplacing,angles,quotes}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{patterns}

\begin{figure}

\begin{tikzpicture}[scale=0.86]

	%%%%%%%%%%%%%%% CONTROL SUBCUBE %%%%%%%%%%%%%%%%% 
	
	% colors
	\fill[pattern=crosshatch,pattern color=black, opacity=0.25] (-1, -1.5) -- (-0.5, -1) -- (-2.25, 0.75) -- (-2.75, 0.25);
	\fill[pattern=crosshatch,pattern color=black, opacity=0.25] (1, -1.5) -- (0.5, -1) -- (2.25, 0.75) -- (2.75, 0.25);
%	\fill[pattern=north west lines,pattern color=black, opacity=0.5] (-0.5, -1) -- (0, -1.5) -- (0.5, -1) -- (0, -0.5);
	
	\fill[color=purple!20!blue!40!white!70] (-2.25, 0.75) -- (-0.5, -1) -- (0, -0.5) -- (0.5, -1) -- (2.25, 0.75) -- (0, 3);
	\fill[color=purple!20!blue!40!white!70] (-2.5, 0.5) -- (0, 3) -- (2.5, 0.5);
	
	\fill[color=white] (-3, 0) -- (0, -3) -- (3, 0); 
	
	% control cube
	\draw[-] (0, -3) -- (-3, 0) -- (0, 3) -- (3, 0) -- (0, -3);
	\draw[dashed] (-3, 0) -- (3, 0);
	\draw[dashed] (-2.5, 0.5) -- (2.5, 0.5);

	
	% talagrand subcubes
	\draw[-] (-2.75, 0.25) -- (-1, -1.5) -- (1.75, 1.25);
	\draw[-] (-2.25, 0.75) -- (0, -1.5) -- (2.25, 0.75);
	\draw[-,line width=0.3mm] (-1.75, 1.25) -- (1, -1.5) -- (2.75, 0.25) -- (0,3) -- (-1.75, 1.25);
		
	% nodes
	\node (0) at (0, -2){$0$};
	\node (1) at (0, 1){$1$};
	\node (talagrand-cube) at (1.15, -0.85){$\bT_{\ell}$};
	
%	\node (blah) at (-3.75, 0){$|x| = \frac{m}{2}$};
%	\node (bleh) at (-4.25, 0.5){$|x| = \frac{m + 0.1\eps\sqrt{m}}{2}$};
	
	\draw[decoration={brace,raise=5pt}, decorate, line width=0.25mm] (-3.05, 0) -- node[left=2pt, align=center, text width = 2.5cm] {\footnotesize $\sbra{\frac{m}{2}, \frac{m + 0.1\eps\sqrt{m}}{2}}$} (-3.05, 0.5);
	
	
	%%%%%%%%%%%%%%%% ACTION SUBCUBES %%%%%%%%%%%%%%%%%
	
	% top
	
	\node (heads) at (5.5, 2.5){\includegraphics[width=1.1cm]{images/quarter-front}};
	\node (bh) at (5.5, 1.5){If $\bb_{\ell} = 1$:};
	
	\fill[color=purple!20!blue!40!white!70] (10, 3) -- (9, 4) -- (8, 3);
	\fill[color=purple!20!blue!40!white!70] (10, 2) -- (9, 1) -- (8, 2);
	
	\draw[-] (9, 1) -- (7.5, 2.5) -- (9, 4) -- (10.5, 2.5) -- (9, 1);
	\draw[dashed] (10, 2) -- (8, 2);
	\draw[dashed] (10, 3) -- (8, 3);
	
	\node() at (9, 3.4){$1$};
	\node() at (9, 2.5){$0$};
	\node() at (9, 1.6){$1$};
	
	% bottom
	
	\node (tails) at (5.5, -2){\includegraphics[width=1.1cm]{images/jersey-quarter-back}};
	\node (bt) at (5.5, -3){If $\bb_{\ell} = 0$:};
	
	\draw[-] (9, -3.5) -- (7.5, -2) -- (9, -0.5) -- (10.5, -2) -- (9, -3.5);	
	\draw[dashed] (10, -2.5) -- (8, -2.5);
	\draw[dashed] (10, -1.5) -- (8, -1.5);
	
	\node() at (9, -1.1){$0$};
	\node() at (9, -2){$0$};
	\node() at (9, -2.9){$0$};
	
	\draw[decoration={brace,raise=5pt}, decorate, line width=0.25mm] (10.5, 3) -- node[right=2pt, align=center, text width = 2.5cm] {\footnotesize $\sbra{\frac{a}{2} \pm c_1\sqrt{a}}$} (10.5, 2);

	
	%%%%%%%%%%%%%%%%%%%% EXTRA GOODIES %%%%%%%%%%%%%%%%
	
	\draw[-latex] (2.35, 0.1) -- (4.5, 2.25);
	\draw[-latex] (2.35, 0.1) -- (4.5, -2.25);
	\node () at (2.35, 0.1) [circle,fill,inner sep=1pt]{};
	
	\node (control) at (0, -4.75){$\zo^{\bC} \equiv \zo^m$};
	\node (action) at (9, -4.75){$\zo^{\bA} \equiv \zo^{a}$};
	
	
	
\end{tikzpicture}

\

\caption*{(a) A draw of $\fyes\sim\Dyes$}

\bigskip

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{tikzpicture}[scale=0.86]

	%%%%%%%%%%%%%%% CONTROL SUBCUBE %%%%%%%%%%%%%%%%% 
	
	% colors
	\fill[pattern= crosshatch,pattern color=black, opacity=0.25] (-1, -1.5) -- (-0.5, -1) -- (-2.25, 0.75) -- (-2.75, 0.25);
	\fill[pattern= crosshatch,pattern color=black, opacity=0.25] (1, -1.5) -- (0.5, -1) -- (2.25, 0.75) -- (2.75, 0.25);
%	\fill[pattern=north west lines,pattern color=black, opacity=0.5] (-0.5, -1) -- (0, -1.5) -- (0.5, -1) -- (0, -0.5);
	
	\fill[color=purple!20!blue!40!white!70] (-2.25, 0.75) -- (-0.5, -1) -- (0, -0.5) -- (0.5, -1) -- (2.25, 0.75) -- (0, 3);
	\fill[color=purple!20!blue!40!white!70] (-2.5, 0.5) -- (0, 3) -- (2.5, 0.5);
	
	\fill[color=white] (-3, 0) -- (0, -3) -- (3, 0); 
	
	% control cube
	\draw[-] (0, -3) -- (-3, 0) -- (0, 3) -- (3, 0) -- (0, -3);
	\draw[dashed] (-3, 0) -- (3, 0);
	\draw[dashed] (-2.5, 0.5) -- (2.5, 0.5);

	
	% talagrand subcubes
	\draw[-] (-2.75, 0.25) -- (-1, -1.5) -- (1.75, 1.25);
	\draw[-] (-2.25, 0.75) -- (0, -1.5) -- (2.25, 0.75);
	\draw[-,line width=0.3mm] (-1.75, 1.25) -- (1, -1.5) -- (2.75, 0.25) -- (0,3) -- (-1.75, 1.25);
		
	% nodes
	\node (0) at (0, -2){$0$};
	\node (1) at (0, 1){$1$};
	\node (talagrand-cube) at (1.15, -0.85){$\bT_{\ell}$};
	
%	\node (blah) at (-3.75, 0){$|x| = \frac{m}{2}$};
%	\node (bleh) at (-4.25, 0.5){$|x| = \frac{m + 0.1\eps\sqrt{m}}{2}$};
	
	\draw[decoration={brace,raise=5pt,}, decorate, line width=0.25mm] (-3.05, 0) -- node[left=2pt, align=center, text width = 2.5cm] {\footnotesize $\sbra{\frac{m}{2}, \frac{m + 0.1\eps\sqrt{m}}{2}}$} (-3.05, 0.5);
	
	
	%%%%%%%%%%%%%%%% ACTION SUBCUBES %%%%%%%%%%%%%%%%%
	
	% top
	
	\node (heads) at (5.5, 2.5){\includegraphics[width=1.1cm]{images/quarter-front}};
	\node (bh) at (5.5, 1.5){If $\bb_{\ell} = 1$:};
	
	\fill[color=purple!20!blue!40!white!70] (10, 2) -- (9, 1) -- (8, 2);
	
	\draw[-] (9, 1) -- (7.5, 2.5) -- (9, 4) -- (10.5, 2.5) -- (9, 1);
	\draw[dashed] (10, 2) -- (8, 2);
	\draw[dashed] (10, 3) -- (8, 3);
	
	\node() at (9, 3.4){$0$};
	\node() at (9, 2.5){$0$};
	\node() at (9, 1.6){$1$};
	
	% bottom
	
	\node (tails) at (5.5, -2){\includegraphics[width=1.1cm]{images/jersey-quarter-back}};
	\node (bt) at (5.5, -3){If $\bb_{\ell} = 0$:};
	
	\fill[color=purple!20!blue!40!white!70] (10, -1.5) -- (9, -0.5) -- (8, -1.5);
	
	\draw[-] (9, -3.5) -- (7.5, -2) -- (9, -0.5) -- (10.5, -2) -- (9, -3.5);	
	\draw[dashed] (10, -2.5) -- (8, -2.5);
	\draw[dashed] (10, -1.5) -- (8, -1.5);
	
	\node() at (9, -1.1){$1$};
	\node() at (9, -2){$0$};
	\node() at (9, -2.9){$0$};
	
	\draw[decoration={brace,raise=5pt}, decorate, line width=0.25mm] (10.5, 3) -- node[right=2pt, align=center, text width = 2.5cm] {\footnotesize $\sbra{\frac{a}{2} \pm c_1\sqrt{a}}$} (10.5, 2);
	
	%%%%%%%%%%%%%%%%%%%% EXTRA GOODIES %%%%%%%%%%%%%%%%
	
	\draw[-latex] (2.35, 0.1) -- (4.5, 2.25);
	\draw[-latex] (2.35, 0.1) -- (4.5, -2.25);
	\node () at (2.35, 0.1) [circle,fill,inner sep=1pt]{};
	
	\node (control) at (0, -4.75){$\zo^{\bC} \equiv \zo^m$};
	\node (action) at (9, -4.75){$\zo^{\bA} \equiv \zo^{a}$};
	
\end{tikzpicture}

\

\caption*{(b) A draw of $\fno\sim\Dno$} 


\caption{The left hand side depicts the control subcube $\zo^{\bC}$ with the terms of the Talagrand DNF, and the right hand side depicts an action subcube $\zo^{\bA}$. The cross-hatched region in the control subcube corresponds to outcomes of the control bits for which the action subcube determines the value of the function  and the dashed lines indicate Hamming weight levels.}
\label{fig:monotone-no}
\end{figure}


==> sections/courseub.tex <==
\section{Coarse Testing}
\label{sec:coarse}

In this section, we prove our results about coarse estimates. To do so, we will use variance as a proxy for distance to constant. 

\begin{lemma}[Folklore] \label{lemma:variance-junta-dist}
	Suppose that $f \isafunc$. Let $m := \max_{J \in \binom{[n]}{k}} \sum_{S \subseteq J} \wh{f}^2(S)$, then 
	\[\frac{1}{4}(1 - m) \leq \dist(f, \calJ_k) \leq (1 - m).\]
\end{lemma}

\begin{proof}
Fix a set $J \subseteq [n]$ of $k$ coordinates and let $g \isafunc$ be a junta on $J$. Note that
		$\E[(f - g)^2] \geq 1 - m$ 
	Since $|f(x) - g(x)| \leq 2$, it follows that
	\[\Pr_{x \sim \bits^n} \left[ f(x) \not = g(x) \right] \geq \frac{1}{4} (1-m)\]
	On the other hand, consider the set $J$ that achieves $m$, and let $g = \sum_{S \subseteq J} \wh{f}(S) \chi_S(x)$. Take $h(x) = \sign(g(x))$ and note that 
	\[ \Pr[h(x) \not = f(x)] \leq \Pr[(g(x) - f(x))^2 \geq 1] \leq 1 - m\]	
	which completes the proof.
\end{proof}

Now note that for a fixed set $J \subseteq [n]$ of size $k$, we have 
	\begin{align*}
		\Ex_{\bx_J \sim \bits^J} \sbra{\Varx_{\by_J\bits^{\overline{J}}}\sbra{f(\bx_{J}, \by_{\overline{J}})}} &= \sum_{S \not \subseteq J} \wh{f}(S)^2.
	\end{align*}
This is a straightforward calculation using Parseval's formula; alternatively, see~Chapters 3 and 4 of~\cite{odonnell-book}.
	
%Since, we can quickly compute the variance of $f$, it essentially suffices to compute the variance of the functions $f(\by \sqcup x)$. 
%
%\orange{
%Just jotting down some things before I go to bed:
%\begin{itemize}
%	\item The algorithm will do the following: 
%	\begin{enumerate}
%		\item First get a good estimate of $\Var[f]$, say via just a Chernoff bound.
%		\item For all $J$ with $|J| = k$, get an unbiased estimator of $\Var_{\bx\sim\bits^{\overline{J}}}[f(\bx \sqcup y)]$. Subtract this from variance to get an unbiased estimator for $m_S$. 
%		\item Iterate over all to find maximum $m_S$, use this to compute distance to junta. 
%	\end{enumerate} 
%\end{itemize}
%}


\subsection{Noising Our Functions}
\label{subsec:coarse-noise}

As before, we apply hold-out noising to our functions. That said, since we are now estimating the variance and not the mean, applying noise could decrease the variance of the function. In particular, the weight at high levels in the Fourier spectrum could become quite small.
To circumvent this, we break up computing the variance into two pieces: Computing the variance from low degree terms and high degree terms. 


\begin{lemma} \label{lemma:variance-noise}
	Given a Boolean function $f\isafunc$ and $\rho := 1-\frac{1}{k}$ for an integer $k$, we have
	\[
%	\Ex_{\bx\sim\bits^J}\sbra{\Varx_{\by\sim\overline{J}}\sbra{f(\bx,\by) - \T^J_{1-\frac{1}{k}}f(\bx,\by)} + \Varx_{\by\sim\overline{J}}\sbra{\T_{1-\frac{1}{k}}^J f(\bx,\by)}}\]
%	\[\in 
%	\sbra{(1\pm \red{TODO})\cdot\Ex_{\bx \sim \bits^J} \sbra{\Varx_{\by\bits^{\overline{J}}}\sbra{f(\bx, \by)}}}.
	\Varx_{\bx\sim\bn}[f(\bx)] 
	\geq 
	\Varx_{\bx\sim\bn}\sbra{f(\bx) - \T_{1-\frac{1}{k}}f(\bx)} + \Varx_{\bx\sim\bn}\sbra{\T_{1-\frac{1}{k}}f(\bx)} 
	\geq 
	\pbra{1-\frac{1}{e}}^2 \Varx_{\bx\sim\bn}[f(\bx)].
	\]
\end{lemma}

\begin{proof}
	
\end{proof}


%For the former, we apply noise and use our estimator. For the latter, we note that this can be computed by simply consider the variance of the queries $f|_{B(x,r)}$.
%\begin{lemma}
%Suppose $f \isafunc$, then 
%	\[\E_{\bx \sim \bits^n} \E_{\by \sim B(\bx,r)} \left[ \left( f(\by) - \E_{\bz \sim B(\bx,r)} \left[ f(\bz) \right] \right)^2 \right] = \sum_{S \subseteq [n]} \wh{f}(S)^2 \]
%\end{lemma}

%\red{
%Shyamal points out that here's a simpler way to get an unbiased estimator for $\Var_{\bx\sim\bits^{\overline{J}}}[f(\bx \sqcup y)]$:
%\begin{itemize}
%	\item You can't just square the function, because you have to subtract the mean. So look at $f - \T^J_{1-1/k}f$ and estimate its variance using the local estimator. 
%	\item Estimate variance of $\T^J_{1-1/k}$ using the local estimator once again. 
%	\item Now add things up!
%\end{itemize}
%}


\subsection{Estimating Our Estimator}
\label{subsec:coarse-differentiation}

Recall that our estimator for $\Var[f]$ from~\Cref{subsec:coarse-estimates} was given by 
\begin{equation} \label{eq:stitch}
	\calE(f|_{B(x,r)}) := \sum_{i=1}^r \alpha_i^{r,N} \sum_{|S|=i} \pbra{\frac{\partial f(x)}{\partial x_S}}^2.
\end{equation}
As such, it suffices to obtain estimates for the quantity 
\[\sum_{|S|=i} \pbra{\frac{\partial f(x)}{\partial x_S}}^2.\]
As in~\Cref{subsec:diff}, we will rely on the ability to compute derivatives of the noise operator. In particular, note that using Parseval's formula, 
\begin{align}
\frac{1}{i!}\Ex_{\bx\sim\bn}\sbra{\frac{d^i}{d\rho^i} (\T_{\sqrt{\rho}} f(x))^2 \bigg|_{\rho=1}} 
&= \frac{1}{i!}\cdot\frac{d^i}{d\rho^i}\pbra{\sum_{T} \rho^{|T|}\wh{f}(T)^2} \bigg|_{\rho=1}	 \nonumber \\ 
&= \sum_{|T|\geq i} \frac{|T|(|T|-1)\cdots(|T|-i+1)}{i!} \wh{f}(T)^2 \nonumber \\ 
&= \Ex_{\bx\sim\bn}\sbra{\sum_{|S|=i} \pbra{\frac{\partial f(\bx)}{\partial x_S}}^2}. \label{eq:coarse-diff-estimator}
\end{align}
Recalling the Leibniz formula, we have 
\begin{equation} \label{eq:leibniz}
	\frac{1}{i!}\cdot{\frac{d^i}{d\rho^i} (\T_{\sqrt{\rho}} f(x))^2} \bigg|_{\rho=1} = \frac{1}{i!}\cdot\sum_{\ell = 0}^i {i\choose \ell} \pbra{ \frac{d^\ell }{d\rho^\ell}\T_{\sqrt{\rho}}f(x) } \cdot \pbra{ \frac{d^{i-\ell}}{d\rho^{i-\ell}}\T_{\sqrt{\rho}}f(x) } \bigg|_{\rho=1}.
\end{equation}
Note that the chain rule allows us to write 
\begin{equation} \label{eq:chain}
	\frac{d}{d\rho}\T_{\sqrt{\rho}}f(x) = \frac{d}{d\upsilon}\T_{\upsilon}f(x) \bigg|_{\upsilon = \sqrt{\rho}} \cdot\frac{d\sqrt{\rho}}{d\rho} = \frac{1}{2\sqrt{\rho}} \cdot \frac{d}{d\upsilon}\T_{\upsilon}f(x) \bigg|_{\upsilon = \sqrt{\rho}}.
\end{equation}

This can be repeatedly iterated, and so~\Cref{eq:leibniz} can be computing using higher derivatives of the usual noise operator $\T_\rho$. We do not derive a closed form expresssion as it seems unweildy. Instead, we record the following lemma:

\begin{lemma}
\label{lem:derivative-expansion}
There exists coefficients such that
	\[ \frac{d^\ell}{d\rho^\ell} (\T_{\sqrt{\rho}} f(x))^2 = \sum_{i = -1}^\ell \sum_{j = -1}^\ell c_{i,j} \frac{d^i}{d\rho^i} T_\rho f \bigg|_{\rho = 1} \cdot \frac{d^j}{d\rho^j} T_\rho f \bigg|_{\rho = 1} \]
where we take $\frac{d^{-1}}{d\rho^{-1}} T_\rho f = 1$. Moreover, we have that $|c_{i,j}| \leq (2 \ell)^{O(\ell)}$
\end{lemma}

\begin{proof}[Sketch of Proof]
The expansion into such a formula is simply the result of applying the Leibniz formula and chain rule iteratively, as described above. \spnote{Check this!} The coefficient bounds, follow from standard bounds on binomial coefficients, noting that $\left| \frac{d^i}{d\rho^i} \frac{1}{\sqrt{\rho}} \right| \leq \ell!$ for $i \leq \ell$, and observing that the chain rule expansion of $\frac{d^\ell}{d\rho^{\ell}}$ has at most $\ell^\ell$ terms.
\end{proof}

Recall now that~\Cref{lem:numerical-diff-noise-op} allows us to obtain good estimates of these higher derivatives.

\begin{lemma}
	Fix a positive integer $\ell$ and assume that $\delta \leq (\ell k)^{-O(1)}$. \spnote{Check that I ported these conditions over correctly} then there exists constants $\beta_{i,j,u,v}$ such that if
	\[\wt{\frac{d^\ell}{d\rho^\ell} (\T_{\sqrt{\rho}} f(x))^2} := \sum_{i = -1}^\ell \sum_{j = -1}^\ell \sum_{u = 0}^{2 \ell - 1} \sum_{v = 0}^{2 \ell - 1} \beta_{i,j,u,v} \T_{1 - u \delta^{r/i}} f(x) \cdot \T_{1 - v \delta^{r/j}} f(x) \bigg|_{\rho = 1}\]
	then
		\[\left| \E[\wt{\frac{d^\ell}{d\rho^\ell} (\T_{\sqrt{\rho}} f(x))^2} - \frac{d^\ell}{d\rho^\ell} (\T_{\sqrt{\rho}} f(x))^2 ] \right| \leq O(\delta^{\ell/100}).\]
	Moreover, we have that $|\beta_{i,j,u,v}| \leq (2 \ell \delta^{-1})^{O(\ell)}$. Finally, for all $x \in \bits^n$, we have that $\wt{\frac{d^\ell}{d\rho^\ell} (\T_{\sqrt{\rho}} f(x))^2} \leq (2 \ell \delta^{-1})^{O(\ell)}$ 
\end{lemma}

\begin{proof}
We simply invoke Lemma \ref{lem:numerical-diff-noise-op} to compute each of the derivative of the noise operator in each term that appears in \Cref{lem:derivative-expansion}. Using the bounds on the size of $\beta$, then follows by the bounds on $|\gamma_i^{\ell, \delta}|$. It's also easy to see that thee bounds on the ceoefficients imply the bounds on the operator $\wt{\frac{d^\ell}{d\rho^\ell} (\T_{\sqrt{\rho}} f(x))^2}$. Finally, statement about the expectation follows by using Cauchy Schwartz to get that
	\[ \E_{\bx} \left [\left( (\wt{\frac{d^\ell}{d\rho^\ell} (\T_{\sqrt{\rho}} f(x))^2} - \frac{d^\ell}{d\rho^\ell} (\T_{\sqrt{\rho}} f(x))^2)^2 \right)^2 \right]  \leq (2\ell)^{100} \cdot (2 \ell \delta^{-1})^{O(\ell)} \delta^{\ell/6}.\]
	This implies the desired claim by \Cref{lem:low-var-expectation}.
\end{proof}


\begin{proposition} \label{prop:coarse-estimating-the-estimator}
	Let $f\isafunc$ be a Boolean function. Suppose $k$ and $r$ are integers where $k$ is sufficiently large. Let $\rho := 1 - \frac{r}{k}$ and $\delta = O(\red{TODO})$ for some parameters $\eps_1,\eps_2$. There exists an $r$-local estimator $\calE^{\star}_{\rho,\delta,r}$ that can be implemented non-adaptively such that 
	\[\Var[\T_\rho f] \geq \Ex_{\bx\sim\bn}\sbra{\calE^{\star}_{\rho,\delta, r}(\T_{\rho}f(\bx)|_{B(\bx,r)})} \geq \red{\text{some function of}}~(r)\cdot\Var[\T_\rho f].\]
\end{proposition}

\begin{proof}
	Let $\calE$ be the coarse estimator from~\Cref{lem:smoothed-coarse-estimator}, i.e. $\calE$ is given by~\Cref{eq:stitch}. Since our noise rate $\rho := 1-\frac{r}{k}$, it follows that 
	\[\bW^{=\ell}[f] \leq \pbra{1- \frac{r}{k}}^{\ell}\bW^{=\ell}[f] \leq \Var[f]\cdot\exp\pbra{-\frac{r\ell}{k}}.\]
	Using~\Cref{lem:smoothed-coarse-estimator} with $t := k/r$ and $K := \Var[f]$, we thus get that there is a $\tau$-local estimator to $\Var[\T_\rho f]$ where 
	\[O\pbra{1 - \Theta\pbra{\frac{r^2}{k\log(k)}}}\Var[\T_\rho f] + O\pbra{\frac{k}{r^2}}\Var[f].\]
	
	We now turn to a description of the estimator $\calE^{\star}_{\rho,\delta,r}$. Let $\alpha_i^{r,N}$ be as in~\Cref{eq:stitch}, and for fixed $i$, let 
	\[
	\wt{\frac{d^i}{d\rho^i}\T_\rho} \qquad\text{be the numerical approximator to}\qquad \frac{d^i}{d\rho^i}\T_\rho
	\]
	given by~\Cref{lem:numerical-diff-noise-op}. We do not give a formal expression for $\calE^\star$, although it is implicitly defined by~\Cref{eq:stitch,eq:coarse-diff-estimator,eq:leibniz,eq:chain}. In particular, we have using~\Cref{eq:leibniz,eq:chain}, there exist coefficients $c_{i,S}$ such that 
	\begin{equation} \label{eq:hairy}
	\sum_{i=1}^r \alpha_i^{r,N} \sum_{|S|=i} \frac{d^i}{d\rho^i} \pbra{\T_{\sqrt{\rho}}f(x)}^2
	=
	\sum_{i=1}^r \alpha_i^{r,N} \cdot \frac{1}{i!} \sum_{S\sse[i]} c_{i,S} \prod_{i\in S} {\frac{d^i}{d\rho^i}\T_\rho}f.
	\end{equation}
	We then define 
	\[
	\calE^{\star}_{\rho,\delta,r}(f) := 
	\sum_{i=1}^r \alpha_i^{r,N} \cdot \frac{1}{i!} \sum_{S\sse[i]} c_{i,S} \prod_{i\in S} \wt{\frac{d^i}{d\rho^i}\T_\rho f}.
	\]
	(It is clear that this estimator can be implemented non-adaptively.)
	Using~\Cref{lem:numerical-diff-noise-op} and following the proof of~\Cref{lem:e-star-good}, one can check\snnote{Check with Shyamal that this actually is correct} that 
	\[\Ex_{\bx\sim\bn}\sbra{\calE^{\star}_{\rho,\delta,r}(\T_\rho f|_{B(\bx,r)})} \in \sbra{\Ex_{\bx\sim\bn}[\calE(\T_\rho f|_{B(\bx,r)})]
	\pm 100r^r\cdot \delta^r/6}.
	\]
	\red{TODO: Is this good enough?}
\end{proof}

%\orange{
%\begin{lemma}
%Let $f \isafunc$, $k$ a sufficiently large positive integer, and $\eps \in (0,\frac{1}{2}]$. Suppose that $r \geq \wt{\Omega}( \sqrt{k \log(1/\eps)})$, $\rho \leq \left(1 - \frac{\sqrt{\log(1/\eps)}}{\sqrt{k}} \right)$, and $\delta \leq O \left( \eps^{12/r} (rk)^{-1000}\right)$, then
%	\[\left | \E_{\bx} \left[ \left| \calE_{\rho, \delta, r}^\star(f, \bx) \right| \right] - \left| \E_{\bx} \left[ f(\bx) \right] \right| \right| \leq \eps\]
%\end{lemma}
%
%\begin{lemma}
%	Fix an integer $\ell$ and a sufficiently large positive integer $k$. Let $f \isafunc$ and let $g = \T_\rho f$ where $\rho \leq 1 - \frac{1}{\red{k}}$. Then for any positive $\delta \leq O((\ell k)^{-100})$, there exists constants $\gamma_1^{\ell \delta}, ..., \gamma^{\ell, \delta}_{2 \ell - 1}$ with $|\gamma_i^{\ell, \delta}| \leq \left( \frac{2\ell}{\delta^{1/3}} \right)^{3\ell}$ such that
%	\[\Ex_{\bx \sim \bits^n} \left[ \left( \sum_{i = 0}^{2 \ell - 1} \gamma_i^{\ell, \delta} \T_{1 - i \delta} g(\bx) - \frac{d^\ell}{d\rho^\ell} \T_\rho g(\bx) \right)^2 \bigg |_{\rho = 1} \right] \leq O(\delta^{\ell/6}).\]
%\end{lemma}
%
%
%\begin{lemma}[] 
%	Suppose $f:\bn\to[-1,1]$ is a bounded Boolean function such that there exists an integer $t$ and a positive number $K$ for which 
%	\[\bW^{=l}[f] \leq K \exp\pbra{-\frac{\ell}{t}}.\]
%	Let $r \leq 2 \sqrt{t}$ be a positive number. Then there exists an $r$-local estimator that $\tau$-approximates $\Var[f]$ such that $\tau := O\pbra{1 - \Theta\pbra{\frac{r}{t\log(rt)}}}\Var[f] + O\pbra{\frac{Kt}{r}}$.
%\end{lemma}
%}


\subsection{Putting Everything Together}
\label{subsec:coarse-alg}


\begin{algorithm}[H]
\addtolength\linewidth{-2em}

\vspace{0.5em}

\textbf{Input:} $f\isafunc$, an integer $k$, and parameters $\eps_1, \eps_2$ \\
\textbf{Output:} An $\frac{\eps_1}{\eps_2}$-multiplicative estimate for $\dist(f, \calJ_k)$

\

\coarsebt($f, \eps$):
\begin{enumerate}
	\item Set parameters
	\[r := \wt{\Theta}(\sqrt{k\eps_1/\eps_2}) \qquad\text{and}\qquad  m := \exp{r}.\]
	\item Construct coordinate oracles $\calF$ as in \Cref{prop:coord-oracles} with error rate $\eps/3$ and failure probability $\frac{1}{k}$.
	\item For each $S\sse\calF$ with $|S| =k$:
	\begin{itemize}
		\item Draw $m$ points $\bx^{(1)},\ldots , \bx^{(m)} \sim \bits^n$ uniformly and independently at random. For each point, compute
	\[\nu_S(\bx^{(i)}) := 1 - \left(\calE^\star_{\rho,\delta,r}(\widetilde{\T}^{S}_{\rho}f(x)|_{B(x,r)}) + (f(x) - \wt{\T}^S_\rho f(x))^2\right)\]
	where $\calE^\star_{p,\delta,r}$ is as in~\Cref{prop:coarse-estimating-the-estimator}.
	\item Set $\bD_S = \frac{1}{m} \sum_i \nu_S(\bx^{(i)})$.
	\end{itemize}
	\item Output ${\max_S |\bD_S|}$.
\end{enumerate}

\caption{Coarse $k$-Junta Distance}
\label{alg:coarse}
\end{algorithm}

We describe the algorithm in~\Cref{alg:coarse}.

\begin{proof}[Proof of~\Cref{thm:coarse-tester}]
	Recall from~\Cref{prop:coord-oracles} that there are at most $\poly(k,1/\eps)$ many coordinate oracles. Fix a set $S\sse\calF$. 
	Using~\Cref{lemma:variance-junta-dist}, we will control the probability that $\calD_S$ differs from $1-\sum_{T\sse S}\wh{f}(T)^2 =  $.
\end{proof}





